Hourglass Automata

In this paper, we define the class of hourglass automata, which are timed automata with bounded clocks that can be made to progress backwards as well as forwards at a constant rate. We then introduce a new clock update for timed automata that allows hourglass automata to be expressed. This allows us to show that language emptiness remains decidable with this update when the number of clocks is two or less. This is done by showing that we can construct a finite untimed graph using clock regions from any timed automaton that use this new update.

==> eptcsdata.tex <==
\providecommand{\firstpage}{175}
\providecommand{\publicationstatus}{Adriano Peron and Carla Piazza (Eds.):\\
Proceedings of the Fifth International Symposium on\\
Games, Automata, Logics and Formal Verification (GandALF 2014)\\
EPTCS 161, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.161.16}{10.4204/EPTCS.161.16}}
\pdfoutput=1

